Efficient Reactive Synthesis Using Mode Decomposition

Developing critical components, such as mission controllers or embedded systems, is a challenging task. Reactive synthesis is a technique to automatically produce correct controllers. Given a high-level specification written in LTL, reactive synthesis consists of computing a system that satisfies the specification as long as the environment respects the assumptions. Unfortunately, LTL synthesis suffers from high computational complexity which precludes its use for many large cases. A promising approach to improve synthesis scalability consists of decomposing a safety specification into smaller specifications, that can be processed independently and composed into a solution for the original specification. Previous decomposition methods focus on identifying independent parts of the specification whose systems are combined via simultaneous execution. In this work, we propose a novel decomposition algorithm based on modes, which consists of decomposing a complex safety specification into smaller problems whose solution is then composed sequentially (instead of simultaneously). The input to our algorithm is the original specification and the description of the modes. We show how to generate sub-specifications automatically and we prove that if all sub-problems are realizable then the full specification is realizable. Moreover, we show how to construct a system for the original specification from sub-systems for the decomposed specifications. We finally illustrate the feasibility of our approach with multiple case studies using off-the-self synthesis tools to process the obtained sub-problems.

==> assumptions.tex <==
\section{Implicit Assumptions and Silent Mission Failures}
\label{sec:assumptions}
%
Temporal task planning using reactive synthesis requires a discrete
description of the goal (and the world in which the system will
operate).
%
Creating discrete domains for complex continuous enivironments
requires introducing assumptions regarding the relation between the
discrete abstraction and the intention in the real world that
typically includes continuous variables.
%
Thus, the objective in the \emph{real world} can be informally
described as ``\Arw implies \Grw'' (where \Arw represents the
assumptions in the real world and \Grw represents the mission goal
in the real world).
%
Reactive synthesis solves this problem by using \emph{discrete} goals
and assumptions $A_D \Into G_D$.
%
The correctness of the solution is based on two additional
assumptions: ``\Arw implies $A_D$'' and ``$G_D$ implies \Grw'', in
other words that the discrete assumptions hold in the real world and
that accomplishing the discrete goals imply accomplising the mission in
the real world.

We refer to \Arw and the last two implications as \emph{implicit
assumptions}.
%
A \textit{silent mission failure} occurs when a system fails to
achieve its goals \Grw but \Arw does not hold either.
%
As a consequence the implication ``\Arw implies \Grw'' is
satisfied, making it impossible for the system user to distinguish if
\Grw holds or if \Arw did not hold.

\subsection{Handling Assumption Violations}
%
We show two scenarios in which we combine temporal task planning and
Stream Runtime Verification
%
\begin{enumerate}[(A)]
\item Flagging assumption violations after a mission concludes in
  order to detect silent failures.
\item Triggering recovery measures online, such as replanning or
  mission abortion, immediately upon an assumption violation using
  quantitative streams in specifications to facilitate plan adjustment
  \footnote{The complete discrete event control problems and
    assumption used to synthesise plans and monitors, and the data
    obtained from the real and simulated flights discussed in this
    section is available at \url{http://mtsa.dc.uba.ar}.}.
\end{enumerate}
%
We now discuss these separately by describing two missions.

\subsubsection{SRV for Offline Monitoring.}
\label{sec:uav:offline}
%
The first mission uses SRV for assumption monitoring and logging.
%
This is a search and rescue mission with a no-fly zone, with the
instruction of landing when the target is found.
%
The monitor processes the incoming events and monitors and logs
assumption violations alongside the associated relevant information,
which can then be used offline for mission post-hoc analysis.

In this mission we monitor two assumptions.
%
The first assumption checks that the UAV never enters the no-fly zone,
and, if it does, measures the degree of violation as the distance
inside the no-fly zone.
%
The second assumption ensures that the area sensed when entering a
zone covers the zone completely.
%

The first assumption can be easily monitored by calculating for each
input position reading, the depth inside the no-fly zone, returning
\HASK{Nothing} if the UAV is not within a forbidden zone.
%

There are several ways one could monitor the second assumption.
%
In this specification we monitor a stronger property that requires the
attitude and position of the vehicle to be within certain bounds.
%
Since these data measurements may carry noise we include in the
monitor specification a filtering phase that implements a first order
low-pass filter.
%
Note that most cameras may require several seconds to capture a high
resolution image, specially on low-end hardware.
%
For this reason, it is necessary to monitor that the filtered attitude
and position is within the required bounds for every instant between
the \formatAction{open\_capture} command and its corresponding
response event, which is the time frame in which a picture is being
taken.
%
Below we show an \hlola specification that encodes both assumptions.

\LOLASPEC{uav1}

\LOLASPEC{uav1b}

%
\noindent The specification imports geometric facilities from
\LOLACODE{\textbf{theory }\textcolor[HTML]{e69e22}{\textbf{Geometry2D}}},
and Haskell libraries
\LOLACODE{\textcolor[HTML]{e69e22}{\textbf{Data.Maybe}}} and
\LOLACODE{\textcolor[HTML]{e69e22}{\textbf{Data.List}}}, and defines
custom datatypes to interpret the data from the UAV, in lines
\linencolor{1--9}.
%
The input streams of this specification, declared in lines
\linencolor{10--16} encompass the state of the UAV, the current target
position, the no-fly zones and the onboard camera events to detect
when a picture is being captured.
%
The output stream \STRNAME{all\_ok\_capturing} declared in line
\linencolor{17} assesses that, whenever the vehicle is taking a
picture, the height, roll and pitch are acceptable and the vehicle is
near the target location.
%
The output stream \STRNAME{flying\_in\_safe\_zones} from line
\linencolor{19} reports if the UAV is flying outside the forbidden
regions.
%
The stream \STRNAME{flying\_in\_poly} in line \linencolor{20}
partially applies the function \HASK{pointInpoly} from the theory
\LIBNAME{Geometry2D} to the current position to find and return the
forbidden region in which the vehicle is flying, if any, using the
Haskell function \HASK{find}.
%
The output stream \STRNAME{depth\_into\_poly} defined in line
\linencolor{23} takes the minimum of the distances between the vehicle
position and every side of the forbidden region inside of which the
vehicle is flying, if any.
%

The intermediate stream \STRNAME{capturing} from line \linencolor{31}
expresses whether the UAV is taking a picture, using the auxiliary
stream \STRNAME{open\_capture} declared in line \linencolor{34}.
%
The streams \STRNAME{filtered\_alt} and \STRNAME{filtered\_pos}
from lines \linencolor{47} and \linencolor{48} represent the location
and altitude of the UAV filtered to reduce noise from the sensors, a
procedure that is implemented generically by the parameterized stream
\STRNAME{filtered\_pos\_component} in line \linencolor{40}.
%
The intermediate stream \STRNAME{near} declared in line
\linencolor{49} takes the distance from the vehicle location to its
target and checks if it is lower than $1$.
%
Finally, the streams \STRNAME{height\_ok}, \STRNAME{roll\_ok}, and
\STRNAME{pitch\_ok} from lines \linencolor{49--51} calculate that the
corresponding attitude of the vehicle is within certain predefined
boundaries.
%

A logger will store the values of all these streams whenever
\STRNAME{all\_ok\_capturing} is \FALSE to detect a silent failure and
allow a post-hoc analysis.
%
\subsubsection{SRV for Online Monitoring and Adaptation.}
\label{sec:uav:hybridadaptation}
%
In the second mission we demonstrate how SRV can be used, beyond
logging, to support remediation actions during the flight by interacting with components
of the UAV controller.
%
% We also showcase how more sophisticated monitoring capabilities of SRV
% describe the overall expected system behavior.
%
We ran an ordered patrol mission (as described in~\cite{Menghi19}) of
three locations with no-fly zones.
%
% We tailored the monitor specifically for fixed-wing UAV.
%

We built a monitor that uses quantitative data to \emph{predict} the
violation of assumptions, enabling the possibility of reacting to
anticipate and avoid the faulty behavior \textit{before} it occurs.
%
To achieve this, the \hlola monitor specification encodes a simplified
non-linear 2D model of a fixed-wing UAV and the full extent of the
waypoint guidance control algorithm of ArduPilot.
%
Part of the input to this monitor includes the current state of the
system (position, attitude, wind) and the list of waypoints for the
current trajectory.
%
The monitor uses this input together with the non-linear model of the
UAV and the guidance control algorithms to produce, by means of
simulation into the future, a prediction of the UAV's flight path.
%

We add an {\em Extended Kalman Filter} (EKF) to estimate in-flight a
parameter $tau$ from the simplified UAV models, helping to diminish
the error in the predicted flight path.
%
Other parameter identification techniques could be used instead (e.g.,
least squares), but we aimed to show \hlola's ability to implement
state-of-the-art estimation algorithms.

The monitor produces an event to indicate that the monitor anticipates
an abnormal situation in the future:
%
\begin{itemize}
\item If the UAV is predicted to hit the target zone but far from its
  center point, then a \formatAction{nearMiss} event is produced.
%
\item If the target zone is to be completely missed, an event
  \formatAction{goFailed} is produced.
%
Our monitor is specified to hold its failure prediction for several
time instants before producing a \formatAction{goFailed}, to allow the
controller to attempt to correct the airspeed.
%
\item Finally, the monitor produces an event
  \formatAction{abnormalDrift} when the predicted distance of the UAV
  to its intended location is beyond a threshold.
\end{itemize}
%

To utilize the output of our predictive monitors, the following three
requirements are added to the mission plan:
\begin{enumerate}[(1)]
\item upon a \formatAction{nearMiss} the UAV should reattempt to visit
  the location immediately,
\item upon a \formatAction{goFailed} the UAV should skip the location
  and move onto the next location to patrol, and
\item upon an \formatAction{abnormalDrift} event, the UAV should abort
  mission and land.
\end{enumerate}
%

We monitor two properties.
%
The first property predicts how close to the center of the target zone
will the UAV pass, so that the UAV controller can either abort the
mission or try to correct the flight path based on the degree of the
error predicted.
%

The second property observes how the UAV is following the planned path
by predicting the estimated time of arrival and total flight distance.
%
A significant difference is likely to be due to wind conditions, which
is not considered by the plan.
%
The monitor uses this estimated arrival time and distance to compute
the speed at which the vehicle is more likely to succeed in closely
following the trajectory, and the controller uses this information to
change the speed of the UAV accordingly.
%

% Both properties require predicting the UAV's behavior with respect to
% a trajectory to follow.
%
%
Below we show the \hlola specification that monitors both assumptions.
%

\LOLASPEC{uav2}
 
\LOLASPEC{uav2b}

The input streams are data about the state of the vehicle at every
instant (\STRNAME{navigation\_data}, \STRNAME{velocity} and
\STRNAME{position}) and its current target destination
(\STRNAME{target} and \STRNAME{target\_dir}).
%

The output stream \STRNAME{intersDistance} of line \linencolor{13}
estimates how far from the target location will the UAV pass,
returning $-1$ if the UAV is actually moving away from the target
location.
%
The output stream \STRNAME{pi\_controller} shown in line
\linencolor{17} is used to control the UAV's airspeed set-point,
taking a reference velocity of $21$ meters per second and an
estimation of the average UAV speed along with the predicted flight
path, generated from the predicted arrival time and flight distance,
which is calculated by the stream \STRNAME{estim\_data}, declared in
line \linencolor{49}.
%
The main idea is that in order to correctly follow the planned path
one must satisfy a constant turn radius assumption, which (for the
UAV) translates into constant ground-speed.
%
When the UAV has tailwind, for a constant airspeed, it will fly at a
faster ground-speed than when it experiences headwind.
%
Controlling the ground-speed around a fixed value (by actuating on the
airspeed set-point) helps following the desired path more accurately.
%

The intermediate stream \STRNAME{kfuStream} shown in line
\linencolor{23} implements the EKF at every instant, and the
intermediate stream \STRNAME{simulated\_guidance} from line
\linencolor{37} simulates the UAV trajectory based on
the current \STRNAME{navigation\_data}, the \STRNAME{tau} (provided by
the EKF and extracted in line \linencolor{35}), a maximum flight time
of $200$ and the target path, given by the list of its waypoints.
%

The function \HASK{simulate\_guidance} from the theory
\LIBNAME{GuidanceTheory} uses a nested specification
\INNERNAME{simuguidance} to simulate the trajectory of the UAV over
the current list of waypoints, which is captured in the input stream
\STRNAME{route}.

\LOLASPEC{simuguidance}

\noindent{}The successive values of \STRNAME{route} are the linear
trajectories that the UAV is expected to go through.
%
The monitor \INNERNAME{simuguidance} will run until the route is
covered or until the \PARAMNAME{maxtime} is exceeded.
%
For every part of the route, \INNERNAME{simuguidance} will spin up a
second level nested specification \INNERNAME{simuinner} to
simulate successive small steps of the flight in a path between two
waypoints.

\LOLASPEC{simuinner1}

\LOLASPEC{simuinner2}

\noindent{}Every execution of \INNERNAME{simuinner} updates the UAV
roll, yaw, and position, the time consumed, and the distance reached
in the simulation step.
%
The nested monitor \STRNAME{simunner} has no input stream
and as a consequence it will execute until \STRNAME{stop\_simulation}
becomes \TRUE.
%
The monitor calculates the trajectory of the UAV updating its
position, distance traveled, roll, and yaw according to simulation
steps of $0.05$ time units.
%
The simulation stops when the \PARAMNAME{maxtime} is reached, or when
the UAV is no longer \LOLACODE{INTRAVEL} and returns the latest state
of the UAV, along with the total time consumed and the information of
whether the maximum time was reached.

%%% Local Variables:
%%% TeX-master: "main.tex"
%%% TeX-PDF-mode: t
%%% End:


==> macros.tex <==
%\usepackage{cesar-llncs}
\NeedsTeXFormat{LaTeX2e}
\RequirePackage{cesar-llncs}[2004/1/27]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Include useful packages. %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%These are insice cesar-llncs
%\RequirePackage{amsmath}
%\RequirePackage{amssymb}
%\RequirePackage{amsthm}
%\RequirePackage{ltlfonts}
%\RequirePackage{xspace}

%for the tables
\RequirePackage{booktabs}
\RequirePackage{multirow}
\RequirePackage{dcolumn}
%for the images
\RequirePackage{graphicx}
%\RequirePackage{xspace}

%for charts
\RequirePackage{pgfplots}
\graphicspath{{figures/plots/}}
\pgfplotsset{compat=1.11}

%\newcommand{\tessla}{TeSSLa\xspace}
%\newcommand{\striver}{Striver\xspace}

\newcommand{\DIST}{\ensuremath{\mathit{dist}}}
\newcommand{\NEXT}{\ensuremath{\mathit{next}}}
\newcommand{\QUEUE}{\ensuremath{Q}}
\newcommand{\REQ}{\ensuremath{\mathbf{req}}}
\newcommand{\RESP}{\ensuremath{\mathbf{resp}}}
\newcommand{\PEN}{\ensuremath{P}}
\newcommand{\WAIT}{\ensuremath{W}}
\newcommand{\MON}{\ensuremath{\mathit{mon}}}
\newcommand{\SRC}{\ensuremath{\mathit{src}}}
\newcommand{\DST}{\ensuremath{\mathit{dst}}}
\newcommand{\TYPE}{\ensuremath{\mathit{type}}}
\newcommand{\STREAM}{\ensuremath{\mathit{stream}}}
\newcommand{\VAL}{\ensuremath{\mathit{val}}}
\newcommand{\MSG}{\ensuremath{\mathit{msg}}}
\newcommand{\NEW}{\ensuremath{\mathit{new}}}
\newcommand{\INPUTS}{\ensuremath{\mathit{inputs}}}
\newcommand{\OUTPUTS}{\ensuremath{\mathit{outputs}}}
\newcommand{\INSTANT}{\ensuremath{\mathit{instantiate}}}
\newcommand{\SIMPLIFY}{\ensuremath{\textsc{Simplify}}}
\newcommand{\Rold}{\ensuremath{R_{\mathit{old}}}}
\newcommand{\ISEAGER}{\ensuremath{\mathit{eager}}}
\newcommand{\ISLAZY}{\ensuremath{\mathit{lazy}}}
\newcommand{\ROUTE}{\ensuremath{\mathit{route}}}
\newcommand{\SEND}{\ensuremath{\mathit{send}}}
%\newcommand{\subf}{\ensuremath{\mathit{sf}}}
\newcommand{\PRUNE}{\ensuremath{\textsc{Prune}}}
\newcommand{\APPEARS}{\ensuremath{\mathit{appears}}}
\newcommand{\DONE}{\ensuremath{\mathit{done}}}
\newcommand{\ISGROUND}{\ensuremath{\mathit{ground}}}
\newcommand{\Evaluate}{\ensuremath{\textsc{Evaluate}}}
\newcommand{\Subst}{\ensuremath{\textsc{Subst}}}
\newcommand{\ovsigma}{\ensuremath{\overline{\sigma}}}
\newcommand{\ovtau}{\ensuremath{\overline{\tau}}}
%\newcommand{\sem}[1]{\llbracket #1\rrbracket}
% \newcommand{\OUTPUT}{\ensuremath{\textit{out}}}
\newcommand \false {\ensuremath{\mathit{false}}}
\newcommand \true {\ensuremath{\mathit{true}}}

\newcommand{\Osem}[1]{\ensuremath{[#1]}}

\newcommand{\Step}{\textsc{Step}}
\newcommand{\Finalize}{\textsc{Finalize}}
\newcommand{\Monitor}{\textsc{Monitor}}
\newcommand{\Propagate}{\textsc{Propagate}}
\newcommand{\Prune}{\textsc{Prune}}

\newcommand{\nablaR}{\ensuremath{\nabla_{\textit{rem}}}}

\newcommand{\Term}{\ensuremath{\mathit{Term}}}
\newcommand{\Vars}{\ensuremath{\mathit{Vars}}}
\newcommand{\simp}{\ensuremath{\mathit{simp}}}

\newcommand{\DELAY}{\ensuremath{\mathit{delay}}}

\newcommand{\IfThenElse}[3]{\ensuremath{\textup{\texttt{if}}\;#1\;\textup{\texttt{then}}\;#2\;\textup{\texttt{else}}\;#3}}

% Feli:
\newcommand{\felitodo}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red]{Matias: #1}}
\newcommand{\felitext}[1]{\todo[inline,linecolor=red,backgroundcolor=red!25,bordercolor=red]{Matias: #1}}
%\newenvironment{changed}{\felitodo{Review this!}\color[HTML]{a61c1c}}{\color{black}}
% Cesar:
\newcommand{\cesartodo}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{Cesar: #1}}
\newcommand{\cesartext}[1]{\todo[inline,linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{Cesar: #1}}
% Mati:
\newcommand{\matitodo}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green]{Mati: #1}}
\newcommand{\matitext}[1]{\todo[inline,linecolor=green,backgroundcolor=green!25,bordercolor=green]{Mati: #1}}
\newenvironment{changed}{\matitodo{Review this!}\color[HTML]{a61c1c}}{\color{black}}


\newcommand{\DefOR}{\ensuremath{\hspace{0.2em}\big|\hspace{0.2em}}}
\newcommand{\TicksOf}{\keyword{ticksOf}}
\newcommand{\delay}{\keyword{delay}}
\newcommand{\shiftS}{\keyword{shift}}
\newcommand{\CV}{\lstinline[language=Striver]{cv}\xspace}
\newcommand{\setS}[1]{\Syntax{\{} #1 \Syntax{\}}}
\newcommand{\valS}[1]{\textsf{(}#1\textsf{)}}
\newcommand{\T}{\ensuremath{\mathbb{T}}\xspace}
\newcommand{\D}{\ensuremath{\mathbb{D}}\xspace}
\newcommand{\Tplus}{\ensuremath{\mathbb{T}^+}\xspace}
\newcommand{\offsetEpsAbs}{\Tplus_{|\epsilon|}}
\newcommand{\UnionS}{\ensuremath{\mathrel{\textsf{U}}}}
\newcommand{\delayS}[1]{\delay{}~#1}

\newcommand{\PrevSsym}{\ensuremath{\textbf{\texttt{<<}}}}
\newcommand{\PrevEqSsym}{\ensuremath{\textbf{\texttt{<\~}}}}
\newcommand{\SuccSsym}{\ensuremath{\textbf{\texttt{>>}}}}
\newcommand{\SuccEqSsym}{\ensuremath{\textbf{\texttt{>\~}}}}
\newcommand{\PrevStt}[1]{\PrevSsym{}#1}
\newcommand{\PrevEqStt}[1]{\PrevEqSsym{}#1}
\newcommand{\SuccStt}[1]{\SuccSsym{}#1}
\newcommand{\SuccEqStt}[1]{\SuccEqSsym{}#1}
\newcommand{\untypedspecialbot}[1]{\ensuremath{\bot_{\text{#1}}}\xspace}
\newcommand{\specialbot}[2]{\untypedspecialbot{#2}}
\newcommand{\outDpos}{\specialbot{\D}{\texttt{+out}}}
\newcommand{\outDS}{\texttt{-out}}
\newcommand{\outDSpos}{\texttt{+out}}
\newcommand{\notickDS}{\Syntax{notick}}
\newcommand{\fullOutT}{\T_{out}}

% Semantics
\definecolor{darkblue}{rgb} {0.200, 0.200, 0.800}
\definecolor{darkred} {rgb} {0.800, 0.200, 0.200}
\definecolor{darkgreen}{rgb}{0.200, 0.800, 0.200}
\newcommand{\colorEv}[2]{\ensuremath{\textcolor{#2}{\llbracket} #1
    \textcolor{#2}{\rrbracket}}}
\newcommand{\colorSigmaEval}[3]{\ensuremath{\colorEv{#1}{#3}_{#2}}}
\newcommand{\colorEvalSigma}[2]{\colorSigmaEval{#1}{\sigma}{#2}}
\newcommand{\colorEvalRho}[2]{\colorSigmaEval{#1}{\rho}{#2}}
\newcommand{\evalTicks}[1]{\colorEvalSigma{#1}{brown}}
\newcommand{\notickD}{\specialbot{\D}{\texttt{notick}}}

\newcommand{\evalTau}[1]{\colorEvalSigma{#1}{darkblue}}
%\newcommand{\evalLola}[1]{\colorEvalRho{#1}{darkgreen}}
\newcommand{\evalLola}[1]{\colorEv{#1}{darkgreen}}

\newcommand{\dom}{\ensuremath{\mathit{dom}}}
\newcommand{\outTneg}{\specialbot{\T}{\texttt{-out}}}
\DeclareMathOperator{\prevOp}{\reserved{prev}}
\DeclareMathOperator{\succOp}{\reserved{succ}}
\newcommand{\Prevop}{\ensuremath{\prevOp\limits_{<}}}
\newcommand{\PrevEq}{\ensuremath{\prevOp\limits_{\leq}}}
\newcommand{\maxT}{\ensuremath{\bar{1}}\xspace}
\newcommand{\minT}{\ensuremath{\bar{0}}\xspace}
\newcommand{\outTpos}{\specialbot{\T}{\texttt{+out}}}
\newcommand{\SuccEq}{\ensuremath{\succOp\limits_{\geq}}}
\newcommand{\Succ}{\ensuremath{\succOp\limits_{>}}}
\newcommand{\evalEsigma}[1]{\evalEsubs{#1}{\sigma}}
\newcommand{\evalEsubs}[2]{\colorSigmaEval{#1}{#2}{darkred}}

\newcommand{\evalE}[1]{\ensuremath{\colorEv{#1}{darkred}}}
\newcommand{\evalO}[1]{\ensuremath{\colorEv{#1}{darkblue}}}
\newcommand{\evalT}[1]{\ensuremath{\colorEv{#1}{brown}}}


\newcommand{\outDneg}{\specialbot{\D}{\texttt{-out}}}
\newcommand{\outT}{\specialbot{\T}{\texttt{-out}}}
\newcommand{\evalSpecsigma}[1]{\colorEvalSigma{#1}{black}}
\newcommand{\Val}{\mathit{V}}
\newcommand{\SY}[1]{\text{\texttt{#1}}}
\newcommand{\PrevEqV}[1]{\SY{(\~}#1\SY{)}}
\newcommand{\PrevV}[1]{\SY{(<}#1\SY{)}}
\newcommand{\SuccEqV}[1]{\SY{(}#1\SY{\~\xspace)}}
\newcommand{\SuccV}[1]{\SY{(}#1\SY{>)}}

% Equivalence
\newcommand{\strequiv}[1]{\equiv_{#1}}
\newcommand{\sigmaequiv}[2]{\equiv_{#1}^{#2}}
\newcommand{\valequiv}[1]{\equiv_{#1}}

\newcommand{\BT}{\ensuremath{\mathbb{T}_b}\xspace}

\newcommand{\Z}{\ensuremath{\mathbb{Z}}\xspace}

% Dependency graph
\newcommand{\ddep}{\rightarrow}
\newcommand{\ddepPres}{\xrightarrow{0}}
\newcommand{\ddepPresStar}{\xrightarrow{\smash{0}}^*}

\newcommand{\ddepPast}{\xrightarrow{-}}
\newcommand{\ddepFut}{\xrightarrow{+}}

% Striver 2 lola transformation
\newcommand{\KWD}[1]{\ensuremath{\textit{#1}}\xspace}
\newcommand{\default}{\KWD{default}}
\newcommand{\limit}{\KWD{limit}}
%\newcommand{\isTicking}{\KWD{isTicking}}
\newcommand{\isTicking}{\KWD{ticks}}
\newcommand{\noalarm}{\KWD{noalarm}}
%\newcommand{\getValue}{\KWD{getValue}}
\newcommand{\getValue}{\KWD{value}}

\newcommand{\partialmap}{\mathrel{\rightharpoondown}}

% Prelims
\newcommand{\none}{\ensuremath{\bot}}
% \newcommand{\tvon}{\ensuremath{\KWD{tv\_on}}}
\newcommand{\tvstatus}{\ensuremath{\KWD{tv\_status}}}
% \newcommand{\colevel}{\ensuremath{\KWD{co2}}}
\newcommand{\on}{\ensuremath{\KWD{on}}}
\newcommand{\off}{\ensuremath{\KWD{off}}}
\newcommand{\typeof}{\KWD{type}}
\newcommand{\maybeGet}{\KWD{maybeGet}}
\newcommand{\len}[1]{\ensuremath{[#1]}}
\newcommand{\bb}{\ensuremath{\tau}}
\newcommand{\tostream}{\KWD{tostream}}
\newcommand{\toseq}{\KWD{toseq}}
\newcommand{\prune}{\KWD{prune}}
\newcommand{\vals}{\KWD{vals}}

\newcommand{\streamvals}{\sigma}
\newcommand{\seqvals}{\rho}
\newcommand{\toLola}{\KWD{lola}}
\newcommand{\toStriver}{\KWD{striver}}

\newcommand{\Reals}{\ensuremath{\mathbb{R}}}
\newcommand{\Rationals}{\ensuremath{\mathbb{Q}}}
\newcommand{\Ints}{\ensuremath{\mathbb{Z}}}

% \newcommand{\shiftAccesses}{\KWD{shiftAcc}}
\newcommand{\shiftAccesses}{\KWD{shift}}
\newcommand{\truestream}{\KWD{true}}
%\newcommand{\shifted}{\KWD{shifted}}
%\newcommand{\expand}{\KWD{expand}}
\newcommand{\expand}{\KWD{exp}}
\newcommand{\nowKW}{\KWD{now}}

% \newcommand{\firstx}{\lstinline[language=Striver,mathescape=true]{first_$x$}}
\newcommand{\firstx}{\verb+first_+$x$}
\newcommand{\lastx}{\verb+last_+$x$}
%\newcommand{\lastx}{\lstinline[language=Striver,mathescape=true]{last_$x$}}

\newcommand{\Time}{\KWD{time}}



\newcommand{\striver}{\textsf{Striver}\xspace}

\newcommand{\tessla}{TeSSLa\xspace}

\newcommand{\reserved}[1]{\ensuremath{\mathit{#1}}\xspace}
\newcommand{\keyword}[1]{\ensuremath{\mathbf{#1}}\xspace}
\newcommand{\Syntax}[1]{\keyword{#1}}

%\newcommand{\URL}{\url{http://github.com/imdea-software}}
\newcommand{\DockerURL}{\url{http://hub.docker.io/imdea-software/rv2020/}}
\newcommand{\hlola}{\textsc{HLola}\xspace}
\newcommand{\lola}{\textsc{Lola}\xspace}
\newcommand{\lvp}{\textit{\TYNAME{LVP}}\xspace}
% \newcommand{\moby}{\fontfamily{pcr}\selectfont MoBy}
\newcommand{\moby}{{\fontfamily{pcr}\selectfont MoBy}\xspace}
\newcommand{\mobi}{\moby}
\newcommand{\gamestructure}{\mathcal{G} = (V, I, O, \theta_e, \theta_s, \psi_e, \psi_s)\xspace}
\newcommand{\hstriver}{HStriver\xspace}

\newcommand{\SLICEDEP}{\ensuremath{\mathit{+^{\hspace{-0.09cm}0}}}\xspace}
% \newcommand{\SLICEEDGE}{\ensuremath{\xrightarrow{\SLICEDEP}}\xspace}
\newcommand{\SLICEEDGE}{\ensuremath{\rightarrow^{+}\xspace}}

\newcommand{\lattice}{\textsf{Lattice}\xspace}

% syntax
\newcommand{\STRNAME}[1]{\texttt{\footnotesize \textcolor[HTML]{eb7600}{\textbf{#1}}}\xspace}
\newcommand{\INNERNAME}[1]{\texttt{\footnotesize \textcolor[HTML]{4d8491}{\textbf{#1}}}\xspace}
\newcommand{\TYNAME}[1]{\texttt{\footnotesize \textcolor[HTML]{008000}{\textbf{#1}}}\xspace}



%\newcommand{\wakeUpTicks}{\reserved{ticks^*}}
%\newcommand{\ticks}{\reserved{ticks}}
%\newcommand{\val}{\reserved{val}}
%
%\newcommand{\caseof}[1]{\mathtt{case}~#1~\mathtt{of}}
%%\newcommand{\IF}{\mathtt{if}}  %% Defined in algorithmic
%%\newcommand{\THEN}{\mathtt{then}}
%%\newcommand{\ELSE}{\mathtt{else}}
%%\newcommand{\ELSIF}{\mathtt{elsif}}
%
%\newcommand{\IfThenElse}[3]{\IF~~#1~~\THEN~~#2~~\ELSE~~#3}
%
%\newcommand{\Not}{\mathclose{\neg}}
%\renewcommand{\And}{\mathrel{\wedge}}
%\newcommand{\Or}{\mathrel{\vee}}
%\newcommand{\Impl}{\mathrel{\rightarrow}}
%\newcommand{\Then}{\mathrel{\rightarrow}} %% ce
%\newcommand{\Iff}{\mathrel{\leftrightarrow}}
%\newcommand{\A}[1]{{\forall #1 \,}}
%%\newcommand{\E}[1]{{\exists #1 \,}}
%\newcommand{\Eu}[1]{{(\exists! #1) \,}}
%
%\newcommand{\Into}{\mathrel{\rightarrow}}
% \newcommand{\IntoP}{\mathrel{\rightharpoondown}}
\newcommand{\IntoP}{\mathrel{\rightharpoonup}}
%
%
%\newcommand{\Nat}{\mathbb{N}}
%\newcommand{\tuple}[1]{\langle#1\rangle} 
%\newcommand{\tupleof}[1]{\langle#1\rangle} 
%
%\newcommand{\default}{\reserved{default}}
%\newcommand{\Time}{\reserved{time}}
%\newcommand{\last}{\reserved{last}}
%\newcommand{\lift}{\reserved{lift}}
%\newcommand{\delay}{\keyword{delay}}
%
%\newcommand{\PrevVal}{\reserved{valprev}}
%%\newcommand{\Prev}{\reserved{tprev^{\leftarrow}}}
%%\newcommand{\Prev}{\reserved{prev}}
%%\DeclareMathOperator*{\prevOp}{\reserved{prev}}
%\DeclareMathOperator{\prevOp}{\reserved{prev}}
%\DeclareMathOperator{\succOp}{\reserved{succ}}
%%\newcommand{\Prev}{\ensuremath{\ensuremath{\reserved{prev}}\limits{\leq}}}
%%\newcommand{\Prev}{\ensuremath{\prevOp\limits_{<}}}
%\newcommand{\PrevEqVal}{\reserved{valprev_\circ}}
%%\newcommand{\PrevEq}{\reserved{tprev}}
%%\newcommand{\PrevEq}{\reserved{prev_\circ}}
%\newcommand{\PrevEq}{\ensuremath{\prevOp\limits_{\leq}}}
%\newcommand{\Succ}{\ensuremath{\succOp\limits_{>}}}
%\newcommand{\SuccEqVal}{\reserved{valsucc_\circ}}
%%\newcommand{\SuccEq}{\reserved{tsucc}}
%%\newcommand{\SuccEq}{\reserved{succ_\circ}}
%\newcommand{\SuccEq}{\ensuremath{\succOp\limits_{\geq}}}
%
%\newcommand{\PrevS}{\Syntax{\ll}}
%%\newcommand{\PrevEqS}{\Syntax{<\sim}}
%%\newcommand{\PrevEqS}{\Syntax{<\text{\raisebox{10ex}{$\sim$}}}}
%%\newcommand{\PrevEqS}{\ensuremath{\mathrel{\ooalign{$<$\cr\hidewidth\raise{20ex}\hbox{$\sim$}\cr}}}}
%\newcommand{\PrevEqS}{\ensuremath{\mathrel{\ooalign{$<$\cr\hidewidth\raisebox{-1.2ex}{$\sim$}\cr}}}}
%\newcommand{\SuccS}{\Syntax{\gg}}
%%\newcommand{\SuccEqS}{\Syntax{\sim>}}
%\newcommand{\SuccEqS}{\ensuremath{\mathrel{\ooalign{$>$\cr\hidewidth\raisebox{-1.2ex}{$\sim$}\cr}}}}
%\newcommand{\setS}[1]{\Syntax{\{} #1 \Syntax{\}}}
%\newcommand{\valS}[1]{\textsf{(}#1\textsf{)}}
%\newcommand{\Ticks}{\keyword{ticks}}
%\newcommand{\ticksS}{\keyword{ticks}}
%\newcommand{\Union}{\mathrel{\textsf{U}}}
%\newcommand{\delayS}[1]{\Syntax{delay (}#1\Syntax{)}}
%
%
%\newcounter{Problem} \setcounter{Problem}{0}
%
%\newcommand{\Prob}{\addtocounter{Problem}{1}\noindent\paragraph{\textbf{Problem
%      \#\theProblem}}}
%
%\newcommand{\Abs}[1]{\ensuremath{#1^\#\xspace}}
%
%\newcommand{\LET}{\mathtt{let}}
%\newcommand{\IN}{\mathtt{in}}
%\newcommand{\MAX}{\ensuremath{\mathit{max}}}
%\newcommand{\DefinedAs}{\ensuremath{\,\stackrel{\text{\textup{def}}}{=}\,}}
%%\newcommand{\DefOr}{\ensuremath{\hspace{1em}\big|\hspace{1em}}}
%\newcommand{\DefOR}{\ensuremath{\hspace{0.2em}\big|\hspace{0.2em}}}
%
%
%\newcommand{\tprev}{\ensuremath{t_{\textit{prev}}}}
%
%\newcommand{\T}{\ensuremath{\mathbb{T}}\xspace}
%\newcommand{\Tstar}{\ensuremath{\mathbb{T}^*}\xspace}
%
%\newcommand{\dom}{\ensuremath{\mathit{dom}}}
%
%%%%%%%%%%%% FROM ANOTHER PAPER ON Nested SRV
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Runtime Verification Macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand{\Clock}{\textit{clock}}
%\newcommand{\Xclock}{\ensuremath{X_\Clock}}
%\newcommand{\Pos}{\ensuremath{\textit{Pos}}}
%\newcommand{\SRV}{SRV\xspace}
%\newcommand{\NRV}{NestedSRV\xspace}
%
%%%%% types
\newcommand{\BoolT}{\textit{Bool}}
\newcommand{\NatT}{\textit{Nat}}
\newcommand{\IntT}{\textit{Int}}
\newcommand{\StackT}{\textit{Stack}}
\newcommand{\SetT}{\textit{Set}}
\newcommand{\ElemT}{\textit{Elem}}
\newcommand{\andsym}{\texttt{and}}
\newcommand{\orsym}{\texttt{or}}
\newcommand{\notsym}{\texttt{not}}
\newcommand{\truesym}{\texttt{true}}
\newcommand{\falsesym}{\texttt{false}}
\newcommand{\SP}{\hspace{0.03em}}
%
\newcommand{\ifthenelsesym}{
  $\begin{bmatrix}
    \sym{if}\SP\cdot\SP\sym{then}\SP\cdot\SP\\
        \hspace{0.12em}\sym{else}\SP\cdot\SP
  \end{bmatrix}$}
\newcommand{\ifthenelsetype}[1]{
  $\begin{array}{l}\BoolT \times #1 \times #1\\
    \hspace{3em}\Into #1
  \end{array}$
}
\newcommand{\BoolName}{\textit{Booleans}}
\newcommand{\BoolSorts}{\BoolT}
\newcommand{\NatName}{\textit{Naturals}}
\newcommand{\NatSorts}{\NatT, \BoolT}
\newcommand{\SetName}{\textit{Sets}}
\newcommand{\SetSorts}{\SetT, \BoolT, \ElemT}
\newcommand{\StackName}{\textit{Stacks}}
\newcommand{\StackSorts}{\StackT, \BoolT, \ElemT}
%
%%%%%%
%
\newcommand{\Sres}{S_{\text{res}}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calF}{\mathcal{F}}
%\newcommand{\Term}{\ensuremath{\textit{Term}}}
%\newcommand{\Expr}{\ensuremath{\textit{Expr}}}
%\newcommand{\NExpr}{\ensuremath{\textit{NestedExpr}}}
%\newcommand{\NestedAtomic}[1]{\ensuremath{\textit{NestedOffset}(#1)}}
%\newcommand{\Atomic}[1]{\ensuremath{\textit{Offset}(#1)}}
%%\newcommand{\In}{\mathcal{I}}
%%\newcommand{\Out}{\mathcal{O}}
%\newcommand{\In}{I}
%\newcommand{\Out}{O}
%\newcommand{\Eqs}{\mathcal{E}}
%\newcommand{\Dom}{\mathcal{D}}
%%\newcommand{\sym}[1]{#1}
%%\newcommand{\sym}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\sym}[1]{\ensuremath{\mathtt{#1}}}
%\newcommand{\symIF}{\sym{if}}
%\newcommand{\symTHEN}{\sym{then}\xspace}
%\newcommand{\symELSE}{\sym{else}\xspace}
%\newcommand{\symTRUE}{\sym{true}\xspace}
%\newcommand{\symFALSE}{\sym{false}\xspace}
\newcommand{\symf}{\sym{f}}
%%\newcommand{\DOM}[1]{{#1}^{\Dom}}
\newcommand{\DOM}[1]{#1}
\newcommand{\domf}{\DOM{f}}
%\newcommand{\clock}[1]{\ensuremath{\text{$#1$}}\xspace}
%\newcommand{\clockn}{\clock{n}}
%\newcommand{\symDIV}{\sym{div}}
%\newcommand{\otau}{\overline{\tau}}
%\newcommand{\osigma}{\overline{\sigma}}
%\newcommand{\anext}[3]{\ensuremath{#1 \leadsto_{#3} #2}}
%
%
%\newcommand{\Pred}{\ensuremath{\textit{pred}}}
%% Language name
%\newcommand{\NSRV}{NestedSRV\xspace}
%\newcommand{\LOLA}{LOLA\xspace}
%
%
%% Translation stuff
%\newcommand{\tigger}{trigger\xspace}
%\newcommand{\tiggers}{triggers\xspace}
%\newcommand{\Tiggers}{Triggers\xspace}
%
%% To change!!!
%\newcommand{\SIC}{\ensuremath{\parallel_{\mathcal{P}}}}
%
%\newcommand{\true}{\text{True}}
%\newcommand{\false}{\textrm{False}}
%
%\newcommand{\ctrue}{\tbf{true}}
%\newcommand{\cfalse}{\tbf{false}}
%
%%\newcommand{\default}{c}
%
%% Specification
%\newcommand{\Spec}{\varphi}
%
%% Input variables
%\newcommand{\iv}{t}
%\newcommand{\ivcall}{\iv_{call}}
%\newcommand{\ivbeg}{\iv_{beg}}
%\newcommand{\ivend}{\iv_{end}}
%\newcommand{\ivret}{\iv_{ret}}
%% Output variable
%\newcommand{\ov}{s}
%% Any stream variable 
%\newcommand{\asv}{v}
%
%
%% Output stream
%\newcommand{\os}{\sigma}
%% Input streams
%\newcommand{\is}{\tau}
%\newcommand{\iscall}{\is_{call}}
%\newcommand{\isbeg}{\is_{beg}}
%\newcommand{\isend}{\is_{end}}
%\newcommand{\isret}{\is_{ret}}
%% Any stream
%\newcommand{\as}{\sigma}
%
%% Abstract sum over execution model
%\newcommand{\asum}[1]{\oplus_{#1}}
%\newcommand{\aminus}[1]{\ominus_{#1}}
%
%% Guess
%%\newcommand{\G}{\mathcal{G}}
%\newcommand{\I}{\mathcal{I}}
%
%\newcommand{\gaprev}[1]{\ensuremath{#1 . \ttt{prev}_{abs}}}
%\newcommand{\gcprev}[1]{\ensuremath{#1 . \ttt{prev}_{con}}}
%\newcommand{\gnow}[1]{\ensuremath{#1 . \ttt{now}}}
%\newcommand{\gcnext}[1]{\ensuremath{#1 . \ttt{next}_{con}}}
%\newcommand{\ganext}[1]{\ensuremath{#1 . \ttt{next}_{abs}}}
%
%% Input
%\newcommand{\inp}{\sigma}
%\newcommand{\Inp}{\Sigma}
%
%% Execution model
%\newcommand{\exm}{\eta}
%\newcommand{\Exm}{H}
%
%% Automata
%\newcommand{\LA}[1]{\mathcal{L}(#1)}
%\newcommand{\Aut}[1]{A}
%
%% Path
%\newcommand{\path}{\alpha}
%
%% Common types
%\newcommand{\FNat}{\Nat_\bot}
%
%% Brackets, tuples
%\newcommand{\Bracket}[1]{\llbracket #1 \rrbracket}
%\newcommand{\Tup}[1]{\ensuremath{\langle #1 \rangle}}
%
%% Felipe's notes
%\newcommand{\felitodo}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red]{Felipe: #1}}
%\newcommand{\felitext}[1]{\todo[inline,linecolor=red,backgroundcolor=red!25,bordercolor=red]{Felipe: #1}}
%
%
%\definecolor{darkblue}{rgb} {0.200, 0.200, 0.800}
%\definecolor{darkred} {rgb} {0.800, 0.200, 0.200}
%\definecolor{darkgreen}{rgb}{0.200, 0.800, 0.200}
%
% \newcommand{\colorEv}[2]{\ensuremath{\textcolor{#2}{\llbracket} #1
%     \textcolor{#2}{\rrbracket}}}
%\newcommand{\colorSigmaEval}[3]{\ensuremath{\colorEv{#1}{#3}_{#2}}}
% \newcommand{\colorEval}[2]{\colorEv{#1}{#2}}
%\newcommand{\colorEvalSigma}[2]{\colorSigmaEval{#1}{\sigma}{#2}}
%%\newcommand{\evalSpec}[1]{\colorSigmaEval{#1}{darkblue}}
% \newcommand{\evalSpec}[1]{\colorEval{#1}{black}}
%\newcommand{\evalSpecsigma}[2]{\colorEval{#1}{#2}{black}}
%\newcommand{\evalE}[1]{\colorEval{#1}{darkred}}
%\newcommand{\evalEsigma}[2]{\colorSigmaEval{#1}{#2}{darkred}}
%%\newcommand{\evalTau}[1]{\colorSigmaEval{#1}{darkgreen}}
%\newcommand{\evalTau}[1]{\colorEvalSigma{#1}{darkblue}}
%\newcommand{\evalTauN}[1]{\colorEval{#1}{darkblue}}
%\newcommand{\evalTausigma}[2]{\colorSigmaEval{#1}{#2}{darkblue}}
%\newcommand{\evalTicks}[1]{\colorEvalSigma{#1}{brown}}
%\newcommand{\evalTicksN}[1]{\colorEval{#1}{brown}}
%\newcommand{\evalTickssigma}[2]{\colorSigmaEval{#1}{#2}{brown}}
%\newcommand{\presentLabel}{\ensuremath{\mathcal{O}}}
%\newcommand{\pastLabel}{\ensuremath{\prec}}
%\newcommand{\edgesSpec}{\ensuremath{Edges_\spec}}
%\newcommand{\interp}{\mathcal{I}}
%
%%\newcommand{\undef}{\reserved{undef}}
%
%\newcommand{\specialbot}[2]{\ensuremath{\bot^{#1}_{\text{#2}}}\xspace}
%\newcommand{\untypedspecialbot}[1]{\ensuremath{\bot_{\text{#1}}}\xspace}
%\newcommand{\D}{D}
%
%% \newcommand{\maybe}[2]{\ensuremath{\mathtt{Maybe}}^#1_{\text{#2}}}
%\newcommand{\outT}{\specialbot{\T}{outside}}
%\newcommand{\outD}{\specialbot{\D}{outside}}
%\newcommand{\notickD}{\specialbot{\D}{notick}}
%\newcommand{\outDS}{\Syntax{outside}_\D}
%\newcommand{\outTS}{\Syntax{outside}_{\T}}
%\newcommand{\notickDS}{\Syntax{notick}_\D}
%\newcommand{\maybe}[2]{\ensuremath{#1 \cup \{\specialbot{#1}{#2}\}}}
%% \newcommand{\outT}{\untypedspecialbot{outside}}
%% \newcommand{\outD}{\untypedspecialbot{outside}}
%% \newcommand{\notickD}{\untypedspecialbot{notick}}
%% \newcommand{\outDS}{\Syntax{outside}}
%% \newcommand{\outTS}{\Syntax{outside}}
%% \newcommand{\notickDS}{\Syntax{notick}}
%
%\newcommand{\maybeOutT}{\maybe{\T}{outside}}
%\newcommand{\maybeOutD}{\maybe{D}{outside}}
%\newcommand{\maybeNotickD}{\maybe{D}{notick}}
%\newcommand{\undef}{\reserved{undef}} % Might be confusing with bottom
%
%\newcommand{\entails}{\vdash}
%\newcommand{\nonZenoT}{2^{\T}_{nz}}
%\newcommand{\offsetEps}{\T_\epsilon}
%
%\newcommand{\lambdatS}[1]{\Syntax{(\text{\textlambda} t . }#1\Syntax{)}}
%\newcommand{\evalAlphaT}[1]{\colorSigmaEval{#1}{black}\alpha_t}
%\newcommand{\evalAlpha}[1]{\colorSigmaEval{#1}{black}\alpha}
%
%%\newcommand{\Val}{\mathcal{V}}
%\newcommand{\Val}{\mathit{V}}
%%\newcommand{\Tau}{\mathit{T}}
%
%
%\newcommand{\Eval}{\mathit{Eval}\xspace}
%\newcommand{\EvalPhi}{\ensuremath{\Eval_\varphi}\xspace}
%
%% Processors
%\newcommand{\colorboxnode}[2]{%
%    \colorlet{currentcolor}{.}%
%    {\color{#1}%
%    \fbox{\color{currentcolor}\strut \ensuremath{#2}}}%
%    \xspace
%}
%\newcommand*{\tickNode}[1]{\colorboxnode{green}{#1}}
%\newcommand*{\valueNode}[1]{\colorboxnode{blue}{#1}}
%\newcommand*{\gateNode}[1]{\colorboxnode{black}{#1}}
%
%\newcommand*{\delayTickNode}{\tickNode{delay}}
%\newcommand*{\srcTickNode}{\tickNode{srcTick}}
%\newcommand*{\constTickNode}{\tickNode{constTick~c}}
%\newcommand*{\UTickNode}{\tickNode{UTick}}
%
%\newcommand*{\prevNode}{\valueNode{prev}}
%\newcommand*{\prevEqNode}{\valueNode{prevEq}}
%\newcommand*{\prevValNode}{\valueNode{prevVal}}
%\newcommand*{\prevEqValNode}{\valueNode{prevEqVal}}
%\newcommand*{\funcNode}{\valueNode{func~f}}
%\newcommand*{\tNode}{\valueNode{\mathbf{t}}}
%
%\newcommand*{\coreNode}{\gateNode{core}}
%\newcommand*{\inputNode}{\gateNode{in}}
%
%\newcommand*{\StreamT}[1]{\ensuremath{\mathcal{S}_{#1}}}
%\newcommand*{\StreamProgressT}[1]{\ensuremath{\mathcal{S}^{\progressEv}_{#1}}}
%\newcommand*{\StreamUnit}{\StreamT{Unit}}
%\newcommand*{\StreamProgressUnit}{\StreamProgressT{Unit}}
%
%% Processor functions
%\newcommand*{\voteFun}{\ensuremath{vote}\xspace}
%\newcommand*{\execFun}{\ensuremath{exec}\xspace}
%\newcommand*{\rinseFun}{\ensuremath{rinse}\xspace}
%\newcommand*{\mayTickFun}{\ensuremath{mayTick}\xspace}
%\newcommand*{\computeValFun}{\ensuremath{computeVal}\xspace}
%
%% Progress events data
%\newcommand*{\progressEv}{\untypedspecialbot{progress}}
%
%% Translation phase
%\newcommand*{\signalFun}{\ensuremath{signalNode}\xspace}
%\newcommand*{\translateTicks}[1]{\ensuremath{translateTicks(#1)}\xspace}
%\newcommand*{\translateSpec}{\ensuremath{translateSpec}\xspace}
%\newcommand*{\translateVal}[1]{\ensuremath{translateVal(#1)}\xspace}
%
%% System state
%\newcommand*{\quiescT}{\ensuremath{\T \cup \{-\infty\}}\xspace}
%\newcommand*{\globalSystem}{\ensuremath{S}\xspace}
%\newcommand*{\graph}{\ensuremath{G}\xspace}
%\newcommand*{\graphT}{\ensuremath{\tupleof{V,E}}\xspace}
%\newcommand*{\eStates}{\ensuremath{\Sigma_E}\xspace}
%\newcommand*{\vStates}{\ensuremath{\Sigma_V}\xspace}
%\newcommand*{\inputTagT}{\ensuremath{InTag}\xspace}
%\newcommand*{\nodeStateT}{\ensuremath{nodeState}\xspace}
%\newcommand*{\edgeStateT}{\ensuremath{edgeState}\xspace}
%\newcommand*{\vStateFunT}{\ensuremath{(V \to \nodeStateT)}\xspace}
%\newcommand*{\eStateFunT}{\ensuremath{(V \times \inputTagT \to \edgeStateT)}\xspace}
%\newcommand*{\dynSys}{\ensuremath{\Sigma}\xspace}
%\newcommand*{\dynSysT}{\ensuremath{\tupleof{\vStateFunT, \eStateFunT}}\xspace}
%\newcommand*{\portTag}[1]{\ensuremath{\mathtt{#1}}\xspace}
%
%% Channel functions
%\newcommand*{\writeChansFun}{\ensuremath{writeChannels}\xspace}
%\newcommand*{\readChansFun}{\ensuremath{readChannels}\xspace}
%\newcommand{\emptyChannel}{\specialbot{\D}{emptychannel}}
%
%% Operational semantics
%\newcommand{\ticksDef}[1]{\mathcal{E}^{ticks}_{#1}}
%\newcommand{\valsDef}[1]{\mathcal{E}^{vals}_{#1}}
%
%
%
%\newcommand{\colorHEval}[2]{\colorSigmaEval{#1}{H}{#2}}
%\newcommand{\evalEH}[1]{\colorHEval{#1}{darkred}}
%\newcommand{\evalTicksH}[1]{\colorHEval{#1}{brown}}
%
%\newcommand{\opEval}[5]{\colorSigmaEval{#4}{#5}{#2\vert_{#1,#3}}(#3)}
%\newcommand{\mayTick}[4]{\opEval{#2}{#3}{#4}{#1}{brown}}
%\newcommand{\computeVal}[4]{\opEval{#2}{#3}{#4}{#1}{darkred}}
%\newcommand{\computeTau}[4]{\opEval{#2}{#3}{#4}{#1}{darkblue}}
%
%% Dependency graph
%\newcommand{\ddep}{\rightarrow}
%\newcommand{\ddepPres}{\xrightarrow{0}}
%\newcommand{\ddepPresStar}{\xrightarrow{\smash{0}}^*}
%
%\newcommand{\ddepPast}{\xrightarrow{-}}
%\newcommand{\ddepFut}{\xrightarrow{+}}
%
%\newcommand{\Present}{\textit{Present}}
%\newcommand{\Past}{\textit{Past}}
%\newcommand{\Future}{\textit{Future}}
%
%%%%% For algorithmic
%
%% New definitions
%\algnewcommand\algorithmicswitch{\textbf{switch}}
%\algnewcommand\algorithmiccase{\textbf{case}}
%\algnewcommand\algorithmicassert{\texttt{assert}}
%\algnewcommand\Assert[1]{\State \algorithmicassert(#1)}%
%% New "environments"
%\algdef{SE}[SWITCH]{Switch}{EndSwitch}[1]{\algorithmicswitch\ #1\ \algorithmicdo}{\algorithmicend\ \algorithmicswitch}%
%\algdef{SE}[CASE]{Case}{EndCase}[1]{\algorithmiccase\ #1}{\algorithmicend\ \algorithmiccase}%
%\algtext*{EndSwitch}%
%\algtext*{EndCase}%
%
%%%%
%\newcommand{\SUP}{\ensuremath{\mathit{sup}}}
%\newcommand{\INF}{\ensuremath{\mathit{inf}}}
%
%\newcommand{\tin}{\ensuremath{t_\textit{in}}}
%%\newcommand{\tqin}{\ensuremath{t_q^{\textit{in}}}}
%\newcommand{\tqin}{\tin}
%\newcommand{\tout}{\ensuremath{t_\textit{out}}}
%%\newcommand{\tqout}{\ensuremath{t_q^{\textit{out}}}}
%\newcommand{\tqout}{\tout}
%\newcommand{\append}{\textit{append}}
%\newcommand{\tq}{\ensuremath{t_q}}
%
%\newcommand{\App}{\ensuremath{\mathrel{\scalebox{0.8}{++}}}}

%\newcommand{\algorithms}[1]{%
%  {\fontfamily{pcr}\selectfont%
%  #1}

%\newcommand{\algorithms}[1]{\texttt{#1}}
% \newcommand{\algo}[1]{#1}

\newcommand{\CM}{\textit{CM}\xspace}
\newcommand{\AP}{\ensuremath{\mathsf{AP}}\xspace}
% %%% LTL
\newcommand{\Always}{\LTLsquare}
\newcommand{\Event}{\LTLdiamond} 
\newcommand{\Next}{\LTLcircle}
\newcommand{\LTLPrev}{\LTLcircleminus}
\newcommand{\PrevNoFirst}{\LTLcircletilde}
\newcommand{\HasAlwaysBeen}{\LTLsquareminus}

\newcommand{\Mode}{\KWD{Mode}}
\newcommand{\mode}{\KWD{mode}}

\newcommand{\VV}{\mathcal{V}}
\newcommand{\VX}{\mathcal{X}}
\newcommand{\VY}{\mathcal{Y}}
\newcommand{\NSF}{\KWD{NSF}}
\newcommand{\jump}{\KWD{jump}}
\newcommand{\done}{\KWD{done}}

\newcommand{\True}{\ensuremath{\text{true}}}
\newcommand{\False}{\ensuremath{\textrm{false}}}
\newcommand{\sv}[1]{\ensuremath{s_{#1}}}
\newcommand{\RemoveTF}{\ensuremath{\textit{remove}\_\textit{tf}\xspace}}
\newcommand{\Simpl}{\ensuremath{\textsc{Simpl}}\xspace}
\newcommand{\NNF}{\KWD{NNF}}
% \newcommand{\NextSF}{\ensuremath{\textsc{next}\_\textsc{sf}\xspace}}
\newcommand{\NextSF}{\ensuremath{\textsc{NextSf}}}
\newcommand{\RmNext}{\ensuremath{\textsc{RmNext}}}
\newcommand{\RmModes}{\ensuremath{\textsc{RmModes}}}
% \newcommand{\Fresh}{\ensuremath{\textsc{Fresh}}}
\newcommand{\Fresh}{\ensuremath{\textsc{Var}}}
\newcommand{\Post}{\ensuremath{\textsc{Post}}}

\newcommand{\Counter}{\KWD{counter}}
\newcommand{\RESET}{\KWD{reset}}
\newcommand{\Trigger}{\KWD{trigger}}

\newcommand{\PR}{\KWD{Pr}}
\newcommand{\Reduce}{\ensuremath{\textsc{Reduce}}}

\newcommand{\ComputeProjections}{\ensuremath{\textsc{ComputeProjection}}}

\newcommand{\Append}{\KWD{append}}
\newcommand{\CurrMode}{\textit{curr}}
\newcommand{\FreshCmode}{\ensuremath{\textit{fresh}\_\textit{cmode}}\xspace}

\newcommand{\Finished}{\textit{finished}}

\newcommand{\subfX}{\ensuremath{\mathit{sub}_{\!X}}}
\newcommand{\Oblig}{\KWD{Oblig}}
\newcommand{\Add}{\KWD{add}}
\newcommand{\subf}{\KWD{sub}}
\newcommand{\Root}{\KWD{root}}
\newcommand{\Compose}{\textsc{Compose}}

